W-RAG: Source-Aware Retrieval for Enterprise Document Generation from Heterogeneous Knowledge Bases

Retrieval-Augmented Generation (RAG) enables large language models to incorporate external knowledge during generation, improving factual grounding and domain adaptability. However, existing RAG pipelines assume that evidence retrieved from multiple repositories can be ranked globally using a single similarity function. While suitable for open-domain retrieval, this assumption breaks down in enterprise document generation, where heterogeneous knowledge bases (such as policies, regulations, technical documentation, and departmental guidelines) serve distinct roles and must be jointly represented in the generated document. As a result, global ranking often produces unbalanced context dominated by a subset of sources, leading to incomplete enterprise drafts. To address this limitation, we propose W-RAG, a source-aware retrieval framework that performs ontology-guided retrieval, local ranking within each knowledge base, and source-level weighting to regulate evidence composition. We further introduce a new dataset for retrieval-grounded enterprise document generation spanning multiple document types and industry domains. Experiments show that standard RAG pipelines struggle on this task, while W-RAG significantly improves document coverage and generation quality.

==> sections/evaluation-metrics.tex <==
\section{Evaluation Metrics}

To comprehensively evaluate the proposed retrieval and generation framework, we combine standard RAG quality metrics with distributional divergence measures that quantify how effectively weighted retrieval influences the composition of the generated response.

\subsection{Standard RAG Quality Metrics}

We first measure semantic correctness and grounding using widely adopted RAG evaluation metrics:

\textbf{Answer Relevancy} evaluates how well the generated response addresses the user query.

\textbf{Faithfulness} measures whether the generated content is supported by the retrieved context, indicating the degree of hallucination or unsupported claims.

\textbf{Context Recall} quantifies how completely the retriever captures relevant supporting information required to answer the query.

These metrics assess the semantic quality of retrieval and generation, answering the question: \emph{Is the retrieved context appropriate and is the generated answer correct and grounded?}

\subsection{Distributional Fidelity Metrics}

Beyond semantic quality, our framework explicitly controls how multiple knowledge sources contribute to the generated response through weighted retrieval. To evaluate whether this compositional intent is preserved, we compare the \emph{target source distribution}
$W=\{W_1,\dots,W_n\}$ produced by the Weight Recommender (C1) with the \emph{realized distribution}
$\hat{W}=\{\hat{W}_1,\dots,\hat{W}_n\}$ obtained via Sentence-Level Attribution (C4).

\paragraph{Chi-Square Statistic}
The chi-square statistic measures systematic deviation between intended and realized source contributions:

\begin{equation}
\chi^2 = \sum_{i=1}^{n} \frac{(W_i - \hat{W}_i)^2}{W_i}.
\end{equation}

This metric highlights sources that consistently over- or under-contribute relative to their assigned weights, enabling detection of unintended dominance from noisy or lower-priority knowledge bases.

\paragraph{Kullback--Leibler Divergence}
KL divergence measures the information loss between the target and realized distributions:

\begin{equation}
D_{\mathrm{KL}}(W \parallel \hat{W}) =
\sum_{i=1}^{n} W_i \log \frac{W_i}{\hat{W}_i}.
\end{equation}

A higher value indicates that the generated response diverges from the intended compositional structure, suggesting that retrieval weighting did not effectively control generation.

\paragraph{Jensen--Shannon Divergence}
Because KL divergence is asymmetric, we additionally compute the Jensen--Shannon divergence, a symmetric and bounded measure:

\begin{equation}
D_{\mathrm{JS}}(W,\hat{W}) =
\frac{1}{2}D_{\mathrm{KL}}(W \parallel M)
+
\frac{1}{2}D_{\mathrm{KL}}(\hat{W} \parallel M),
\end{equation}

where $M=\frac{1}{2}(W+\hat{W})$.

JS divergence provides a stable and interpretable estimate of distributional mismatch, making it suitable for comparing compositional fidelity across experiments.

\subsection{Interpretation}

While Answer Relevancy, Faithfulness, and Context Recall evaluate \emph{semantic correctness}, the divergence-based metrics evaluate \emph{compositional control}. Together, they provide a dual-perspective assessment:

\begin{itemize}
\item \textbf{Semantic quality:} Is the answer correct and grounded?
\item \textbf{Distributional fidelity:} Did weighted retrieval shape which sources contributed to the response?
\end{itemize}

This combined evaluation allows us to verify not only that the system retrieves relevant evidence, but also that it respects the intended balance among knowledge sources enforced by components C1--C3 and measured via C4.

